How Hard is Weak-Memory Testing?

Weak-memory models are standard formal specifications of concurrency across hardware, programming languages, and distributed systems. A fundamental computational problem is consistency testing: is the observed execution of a concurrent program in alignment with the specification of the underlying system? The problem has been studied extensively across Sequential Consistency (SC) and weak memory, and proven to be NP-complete when some aspect of the input (e.g., number of threads/memory locations) is unbounded. This unboundedness has left a natural question open: are there efficient parameterized algorithms for testing? The main contribution of this paper is a deep hardness result for consistency testing under many popular weak-memory models: the problem remains NP-complete even in its bounded setting, where candidate executions contain a bounded number of threads, memory locations, and values. This hardness spreads across several Release-Acquire variants of C11, a popular variant of its Relaxed fragment, popular Causal Consistency models, and the POWER architecture. To our knowledge, this is the first result that fully exposes the hardness of weak-memory testing and proves that the problem admits no parameterization under standard input parameters. It also yields a computational separation of these models from SC, x86-TSO, PSO, and Relaxed, for which bounded consistency testing is either known (for SC), or shown here (for the rest), to be in polynomial time.

==> app_lower_bounded_values.tex <==
\section{Proofs from \cref{SEC:BOUNDED_VALUES}}\label{SEC:APP_BOUNDED_VALUES}

\lemboundedvaluesXOne*
\begin{proof}
We outline a generic argument that works for all memory models in the lemma statement.
Let $\expartial$ be any of the abstract executions $\expartial^{\ramm}$ and $\expartial^{\rlxmm}$, and $\expartial_1$ the corresponding abstract execution $\expartial_1^{\ramm}$ or $\expartial_1^{\rlxmm}$.
Note that all events that are present in $\expartial_1$ but not $\expartial$ access values that are not present in $\expartial$.
Hence, if $\expartial_1$ is consistent in its respective model, so is $\expartial$.

For the opposite direction, let $\ex=(\E, \po, \rf, \mo)$ be any execution that witnesses the consistency of $\expartial$ in any of its respective memory models $\MemModel$.
We construct an execution $\ex_1=(\E_1, \po_1, \rf_1, \mo_1)$ that witnesses the consistency of $\expartial_1$ in $\MemModel$.
In particular, we will specify $\rf^1$ and a partial modification order $\mopartial_1$ that is minimally coherent (for both $\sramm$ and $\rlxmm$).
First, we let $\rf_1\subseteq \rf$ and $\mo_1\subseteq \mopartial_1$.

Second, we describe the $\rf_1$ and $\mopartial_1$ relations concerning events in the blocks $\Block^i_j(x)$.
For each read $\rd(t, x)$ of $\Block^i_j(x)$, we let $(\wt(t',x), \rd(t,x))\in \rf_1$, where $\wt(t',x)$ is the unique write of $\Block^i_j(x)$ accessing the same value as $\rd(t,x)$.
Moreover, for any two writes $\wt(t,x)$ and $\wt(t', x)$ of $\Block^i_j(x)$ with $t\leq_{\sigma_2}t'$, we have $(\wt(t,x), \wt(t',x))\in \mopartial_1$.
In addition, for every write $\wt(t,x)$ of $\Block^i_j(x)$ and conflicting write $\wt(t', x)$ that does not appear in $\Block^i_j(x)$.
Thus $\wt(t',x)$ appears 
(i)~in a copy gadget $\CopyGadget{i'}{j'}$, or
(ii)~in a copy-down gadget $\CopyGadgetDown{i'}{j'}$, or
(iii)~in a block $\Block^{i'}_{j'}(x)$.
If $i'>i$ or $i'=i$ and $j'>j$, then we have $(\wt(t,x), \wt(t',x))\in \mopartial_1$, while if $i'<i$ or $i'=i$ and $j'<j$, then we have $(\wt(t',x), \wt(t,x))\in \mopartial_1$.

Third, we describe the $\rf_1$ and $\mopartial_1$ relations concerning events in the blocks $\Block^i(x)$.
The construction is very similar to the events of the blocks $\Block^i_j(x)$.
In particular, for each read $\rd(t, x)$ of $\Block^i(x)$, we let $(\wt(t',x), \rd(t,x))\in \rf_1$, where $\wt(t',x)$ is the unique write of $\Block^i(x)$ accessing the same value as $\rd(t,x)$.

Moreover, for any two writes $\wt(t,x)$ and $\wt(t', x)$ of $\Block^i(x)$ with $t\leq_{\sigma_2}t'$, we have $(\wt(t,x), \wt(t',x))\in \mopartial_1$.
In addition, for every write $\wt(t,x)$ of $\Block^i(x)$ and conflicting write $\wt(t', x)$ that does not appear in $\Block^i(x)$.
Thus $\wt(t',x)$ appears 
(i)~in an at-most-one-true gadget $\AtMostOneGadget{c}{i}{j}{k}$, or
(ii)~in an at-least-one-true gadget $\AtLeastOneGadget{i}{j}{k}{\ell}$, or
(iii)~in a block $\Block^{i'}(x)$.
If $i'>i$  then we have $(\wt(t,x), \wt(t',x))\in \mopartial_1$, while if $i'<i$ then we have $(\wt(t',x), \wt(t,x))\in \mopartial_1$.

It is not hard to see that $\mopartial_1$ is minimally coherent for both $\sramm$ and $\rlxmm$, though we will not prove this here.
\end{proof}


\lemboundedvaluesXOne*
\begin{proof}
We outline a generic argument that works for all memory models in the lemma statement.
Let $\expartial_1$ be any of the abstract executions $\expartial_1^{\ramm}$ and $\expartial_1^{\rlxmm}$, and $\expartial_2$ the corresponding abstract execution $\expartial_2^{\ramm}$ or $\expartial_2^{\rlxmm}$.
Since every pair of conflicting events that access the same value in $\expartial_1$ also access the same value in $\expartial_2$, if $\expartial_1$ is consistent in one of its respective memory models, so is $\expartial_2$, sharing the same witnessing reads-from relations and modification order.

For the opposite direction, it is straightforward to verify that, due to the blocks $\Block^i_j(x)$ and $\Block^i(x)$ in $\expartial_2$,
every read is forced to read from a write that appears in the same gadget.
But then this read-write pair accesses the same value also in $\expartial_1$, thus the reads-from relation and modification order that witness the consistency of $\expartial_2$ also witness the consistency of $\expartial_1$.

The desired result follows.
\end{proof}

